An LSTM approach to Forecast Migration using Google Trends

Being able to model and forecast international migration as precisely as possible is crucial for policymaking. Recently Google Trends data in addition to other economic and demographic data have been shown to improve the forecasting quality of a gravity linear model for the one-year ahead forecasting. In this work, we replace the linear model with a long short-term memory (LSTM) approach and compare it with two existing approaches: the linear gravity model and an artificial neural network (ANN) model. Our LSTM approach combined with Google Trends data outperforms both these models on various metrics in the task of forecasting the one-year ahead incoming international migration to 35 Organization for Economic Co-operation and Development (OECD) countries: for example the root mean square error (RMSE) and the mean average error (MAE) have been divided by 5 and 4 on the test set. This positive result demonstrates that machine learning techniques constitute a serious alternative over traditional approaches for studying migration mechanisms.

==> tex/models.tex <==
%We use the LSTM approach from \cite{gersLearningForgetContinual2000} which introduced a forget gate to the standard version \cite{hochreiterLongShorttermMemory1997}. 
%This is also the one implemented by the Keras neural network library, which we use in this work \cite{chollet2015keras}. 

As described in figure~\ref{fig:unfolded_lstm} we use one RNN in charge of predicting the bilateral flows $\hat{T}_{i,j}$ with the origin and destination countries one hot encoded for all pairs $(i,j)$.  
The RNN has a unique LSTM layer.
Another approach would have been to use different networks to estimate the flow for each pair of countries. The amount of data to train each would have been very limited, though.


\subsection{Learning models and hyper-parameter optimization}

To train the ML models we proceed using three sets~\cite{goodfellowDeepLearning2016}: (a) a train set, gathering the input features from 2004 to 2012 (input \_features$_{i,j,04..12}$ $\forall i,j$) and also all the observed migration flows spanning from 2005 to 2013 as output (T$_{i,j,05..13}$ $\forall i,j$) since we predict next year migration; (b) a validation set, containing input features on the year 2013 (input\_features$_{i,j,13}$ $\forall i,j$) and migration flows of 2014 (T$_{i,j,14}$ $\forall i,j$); and (c) a test set, on the year 2014 (input\_features$_{i,j,14}$ $\forall i,j$) and 2015 (T$_{i,j,15}$ $\forall i,j$). The hyperparameters are optimized accordingly for each model.

A simplified version of our LSTM training is presented in Algorithm~\ref{alg:train_model}, while our LSTM evaluation is presented in Algorithm~\ref{alg:validation_test_model}. Notice that the span of years presented in the algorithms corresponds to the one used once the validation is completed, i.e., we fit our model on both the training and validation set.

\begin{algorithm}
     \KwData{\textit{model} : LSTM untrained model}
     \KwResult{Model is trained}
     \For{each epoch}{
        \For{each pair i,j of origin-destination countries}{
            \tcc{gradient descent for each batch:}
            \textit{model}.fit(input\_features$_{i,j,04..13}$ , T$_{i,j,05..14}$)
        }
     }
    evaluation(\textit{model}) \tcc{see algorithm 2}
     \caption{Our training algorithm}
     \label{alg:train_model}
\end{algorithm}

\begin{algorithm}
% \Fn(\tcc*[h]{algorithm as a recursive function}){\FRecurs{some args}}{
     \KwData{\textit{model} : LSTM trained model }
     \KwResult{Model is evaluated}
     \For{each pair i,j of origin-destination countries}{
        $\hat{T}_{i,j,15}$ $\leftarrow$ \textit{model}.predict(input\_features$_{i,j,04..14}$) \\
        error $\leftarrow$ compute\_metrics($T_{15}$,$\hat{T}_{15}$)
     }
     \caption{Our evaluation algorithm}
     \label{alg:validation_test_model}
\end{algorithm}

Due to the specificity of LSTM, we fit our LSTM time series by time series\footnote{By time series we mean sequence of annual migration flows between a pair of origin destination.}.
Therefore we use a batch of size corresponding to the number of years present in the serie. This implies that the gradient descent is applied and the LSTM's parameters are updated after each propagation of a time series through the LSTM cells (as presented in figure~\ref{fig:unfolded_lstm}).
Furthermore the features have been normalized by time series of origin destination using a min max scaler~\cite{goodfellowDeepLearning2016}. Our LSTM model uses a bias of 1 for the LSTM forget gate since it has been shown to improve performances drastically~\cite{gersLearningForgetContinual2000,jozefowiczEmpiricalExplorationRecurrent2015}. 

We make use of dropout regularization to reduce the overfitting for both models and ensure a better generalization~\cite{srivastavaDropoutSimpleWay2014,galTheoreticallyGroundedApplication2016,arpitCloserLookMemorization2017}

For the experiments, we have used three different loss functions: Mean Absolute Error ($MAE$), Mean Square Error ($MSE$), and Common Part of Commuters ($CPC$, as described in \cite{robinsonMachineLearningApproach2018}, equivalent to $1 - cpc$ with cpc given by equation \eqref{eq:cpc} ) and adapt them to handle time series.

We optimize the following hyperparameters and present them along with their optimal value : loss function - \textit{MAE} using \textit{adam} optimizer, number and size of hidden layers - \textit{1} layer of width \textit{50}, number of epochs - \textit{50}, and dropout - \textit{0.15}. 

